Marginal Price Optimization

We introduce a new framework for optimal routing and arbitrage in AMM driven markets. This framework improves on the original best-practice convex optimization by restricting the search to the boundary of the optimal space. We can parameterize this boundary using a set of prices, and a potentially very high dimensional optimization problem (2 optimization variables per curve) gets reduced to a much lower dimensional root finding problem (1 optimization variable per token, regardless of the number of the curves). Our reformulation is similar to the dual problem of a reformulation of the original convex problem. We show our reformulation of the problem is equivalent to the original formulation except in the case of infinitely concentrated liquidity, where we provide a suitable approximation. Our formulation performs far better than the original one in terms of speed - we obtain an improvement of up to 200x against Clarabel, the new CVXPY default solver - and robustness, especially on levered curves.

==> _img/arb_tbl_3_tradinstr_r4b.tex <==

\begin{table}[htbp]  % h: here, t: top, b: bottom, p: page
\centering
\small

\begin{tabular}{lrr}
\toprule
{} &     WETH &     USDC \\
\midrule
\textbf{PRICE    } &  1,800.0 &      1.0 \\
\textbf{Lev1     } &    0.018 &  -44.947 \\
\textbf{Lev2     } &   -0.018 &   27.268 \\
\textbf{AMMIn    } &    0.018 &   27.268 \\
\textbf{AMMOut   } &   -0.018 &  -44.947 \\
\textbf{TOTAL NET} &    0.000 &  -17.680 \\
\bottomrule
\end{tabular}


\caption{Trade instruction r4b TODO}
\label{tbl:3_tradinstr_r4b}
\end{table}


==> _img/arb_tbl_3_tradinstr_r4o.tex <==

\begin{table}[htbp]  % h: here, t: top, b: bottom, p: page
\centering
\small

\begin{tabular}{lrr}
\toprule
{} &     WETH &     USDC \\
\midrule
\textbf{PRICE    } &  1,800.0 &      1.0 \\
\textbf{Lev1o    } &    0.036 &  -89.447 \\
\textbf{Lev2o    } &   -0.077 &  115.486 \\
\textbf{AMMIn    } &    0.036 &  115.486 \\
\textbf{AMMOut   } &   -0.077 &  -89.447 \\
\textbf{TOTAL NET} &   -0.041 &   26.039 \\
\bottomrule
\end{tabular}


\caption{Trade instruction r4o TODO}
\label{tbl:3_tradinstr_r4o}
\end{table}


==> _img/arb_tbl_4_curves1.tex <==

\begin{table}[htbp]  % h: here, t: top, b: bottom, p: page
\centering
\small

\begin{tabular}{lrrrrrr}
\toprule
{} &       Pair &    Price & Base Price & Deviation &          L &       L\_USD \\
\textbf{cid} &            &          &            &           &            &             \\
\midrule
\textbf{C00} &  TKN6/TKN3 &   8.1411 &          8 &      1.8\% &     46,341 &   1,048,576 \\
\textbf{C01} &  TKN6/TKN3 &   8.0320 &          8 &      0.4\% &     46,341 &   1,048,576 \\
\textbf{C02} &  TKN0/TKN2 &   0.2524 &        1/4 &      1.0\% &    524,288 &   1,048,576 \\
\textbf{C03} &  TKN4/TKN3 &   2.0448 &          2 &      2.2\% &     92,682 &   1,048,576 \\
\textbf{C04} &  TKN3/TKN2 &   2.0374 &          2 &      1.9\% &    185,364 &   1,048,576 \\
\textbf{C05} &  TKN3/TKN2 &   1.9805 &          2 &     -1.0\% &    185,364 &   1,048,576 \\
\textbf{C06} &  TKN4/TKN1 &   8.0760 &          8 &      1.0\% &    185,364 &   1,048,576 \\
\textbf{C07} &  TKN4/TKN1 &   7.9879 &          8 &     -0.2\% &    185,364 &   1,048,576 \\
\textbf{C08} &  TKN2/TKN1 &   1.9979 &          2 &     -0.1\% &    370,728 &   1,048,576 \\
\textbf{C09} &  TKN6/TKN0 &  64.2628 &         64 &      0.4\% &    131,072 &   1,048,576 \\
\textbf{C10} &  TKN4/TKN2 &   4.0058 &          4 &      0.1\% &    131,072 &   1,048,576 \\
\textbf{C11} &  TKN4/TKN5 &   0.5073 &        1/2 &      1.5\% &     46,341 &   1,048,576 \\
\textbf{C12} &  TKN6/TKN4 &   4.0304 &          4 &      0.8\% &     32,768 &   1,048,576 \\
\textbf{C13} &  TKN1/TKN2 &   0.5006 &        1/2 &      0.1\% &    370,728 &   1,048,576 \\
\textbf{C14} &  TKN0/TKN5 &   0.0314 &       1/32 &      0.4\% &    185,364 &   1,048,576 \\
\textbf{C15} &  TKN0/TKN5 &   0.0314 &       1/32 &      0.3\% &    185,364 &   1,048,576 \\
\textbf{C16} &  TKN2/TKN3 &   0.5075 &        1/2 &      1.5\% &    185,364 &   1,048,576 \\
\textbf{Ca0} &  TKN1/TKN2 &   0.5000 &        1/2 &     -0.0\% &  2,621,440 &   7,414,552 \\
\textbf{Ca1} &  TKN2/TKN3 &   0.5000 &        1/2 &      0.0\% &  3,707,276 &  20,971,520 \\
\textbf{Ca2} &  TKN3/TKN4 &   0.5000 &        1/2 &      0.0\% &  3,707,276 &  41,943,040 \\
\textbf{CaX} &  TKN1/TKN4 &   0.1500 &        1/8 &     20.0\% &  1,853,638 &  10,485,760 \\
\bottomrule
\end{tabular}


\caption{Curves incl arbitrage curves}
\label{tbl:4_curves1}
\end{table}


==> _img/arb_tbl_4_instra.tex <==

\begin{table}[htbp]  % h: here, t: top, b: bottom, p: page
\centering
\small

\begin{tabular}{lrrrr}
\toprule
{} &      TKN1 &     TKN2 &     TKN3 &     TKN4 \\
\midrule
\textbf{PRICE    } &      0.54 &     1.00 &     1.94 &     3.82 \\
\textbf{Ca0      } &  -141,173 &   73,381 &       &       \\
\textbf{Ca1      } &        &  -80,385 &   40,818 &       \\
\textbf{Ca2      } &        &       &  -40,818 &   20,569 \\
\textbf{CaX      } &   141,173 &       &       &  -20,569 \\
\textbf{AMMIn    } &   141,173 &   73,381 &   40,818 &   20,569 \\
\textbf{AMMOut   } &  -141,173 &  -80,385 &  -40,818 &  -20,569 \\
\textbf{TOTAL NET} &         0 &   -7,004 &        0 &        0 \\
\bottomrule
\end{tabular}


\caption{Trade instructions with arbitrage curves only}
\label{tbl:4_instra}
\end{table}


==> _img/arb_tbl_5_diagram.tex <==

\begin{table}[htbp]  % h: here, t: top, b: bottom, p: page
\begin{center}
\begin{tikzcd}
    T \arrow[r, leftrightarrow] & \arrow[d] \varphi \arrow[r, leftrightarrow]  & \arrow[d] \mathcal{G}\\
    & \hat{\varphi} \arrow[r, leftrightarrow] & \hat{\mathcal{G}} \\
\end{tikzcd}
\end{center}
\caption[Transaction representations]{Transaction representations (operator $T$, flow $\varphi$ and graph $\mathcal{G}$; first row is curve level, second row is token level)}
\label{tbl:5_diagram}
\end{table}

